Progress and perspectives on composite laser-pulses spectroscopy for high-accuracy optical clocks

Probing an atomic resonance without disturbing it is an ubiquitous issue in physics. This problem is critical in high-accuracy spectroscopy or for the next generation of atomic optical clocks. Ultra-high resolution frequency metrology requires sophisticated interrogation schemes and robust protocols handling pulse length errors and residual frequency detuning offsets . This review reports recent progress and perspective in such schemes, using sequences of composite laser-pulses tailored in pulse duration, frequency and phase, inspired by NMR techniques and quantum information processing. After a short presentation of Rabi technique and NMR-like composite pulses allowing efficient compensation of electromagnetic field perturbations to achieve robust population transfers, composite laser-pulses are investigated within Ramsey's method of separated oscillating fields in order to generate non-linear compensation of probe-induced frequency shifts. Laser-pulses protocols such as Hyper-Ramsey (HR), Modified Hyper-Ramsey (MHR), Generalized Hyper-Ramsey (GHR) and hybrid schemes are reviewed. These techniques provide excellent protection against both probe induced light-shift perturbations and laser intensity variations. More sophisticated schemes generating synthetic frequency-shifts are presented. They allow to reduce or completely eliminate imperfect correction of probe-induced frequency-shifts even in presence of decoherence due to the laser line-width. Finally, two universal protocols are presented which provide complete elimination of probe-induced frequency shifts in the general case where both decoherence and relaxation dissipation effects are present by using exact analytic expressions for phase-shifts and the clock frequency detuning. These techniques might be applied to atomic, molecular and nuclear frequency metrology, mass spectrometry as well as precision spectroscopy.

==> Figure_IV-Composite-Pulses-Parameters-Dissipation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Figure - Layout
\begin{figure}[t!!]
	\center
	\resizebox{\linewidth}{!}{
		\includegraphics[angle=0]{IV-Composite-Pulses-Parameters-Dissipation}
	}
	\caption{
		Optical pulses are defined by generalized area $\theta_{l}$ ($l=\textup{1,2..,k,..,n}$), frequency detuning $\delta_{l}$,
		field amplitude $\Omega_{l}e^{i\varphi_{l}}$ with phase-step modulation $\varphi_{l}$, pulse duration $\tau_{l}$ and a
		single free evolution time T applied somewhere at the desired $l=\textup{k}$ pulse. Laser-induced decoherence is called
		$\gamma_{c}$, relaxation by spontaneous	emission is labeled $\Gamma$ and $\xi$ is the relaxation rate of population
		difference due to collisions.
	}
	\label{fig:IV-Composite-Pulses-Parameters-Dissipation}
\end{figure}


